Optimal Resource Allocation for Elastic and Inelastic Jobs

Modern data centers are tasked with processing heterogeneous workloads consisting of various classes of jobs. These classes differ in their arrival rates, size distributions, and job parallelizability. With respect to paralellizability, some jobs are elastic, meaning they can parallelize linearly across many servers. Other jobs are inelastic, meaning they can only run on a single server. Although job classes can differ drastically, they are typically forced to share a single cluster. When sharing a cluster among heterogeneous jobs, one must decide how to allocate servers to each job at every moment in time. In this paper, we design and analyze allocation policies which aim to minimize the mean response time across jobs, where a job's response time is the time from when it arrives until it completes. We model this problem in a stochastic setting where each job may be elastic or inelastic. Job sizes are drawn from exponential distributions, but are unknown to the system. We show that, in the common case where elastic jobs are larger on average than inelastic jobs, the optimal allocation policy is Inelastic-First, giving inelastic jobs preemptive priority over elastic jobs. We obtain this result by introducing a novel sample path argument. We also show that there exist cases where Elastic-First (giving priority to elastic jobs) performs better than Inelastic-First. We then provide the first analysis of mean response time under both Elastic-First and Inelastic-First by leveraging recent techniques for solving high-dimensional Markov chains.

==> overview.tex <==
\section{Overview}
We consider a system where jobs of two types arrive over time into a system consisting of $k$ servers.
The first type of job, which we call \textbf{inelastic}, can run on any server, but can only run on one server at any moment in time.
We will assume that inelastic jobs arrive according to a Poisson Process with rate $\lambda_I$. We use the random variable $S_I$ to denote the size of an inelastic job,
The second type of job, called \textbf{elastic}, can run on any server, and can run on \emph{any number} of servers at any moment in time.
Elastic jobs arrive into the system according to a Poisson Process of rate $\lambda_E$. This process is independent of the inelastic arrival process.
Every job has an associated \emph{size} which represents the amount of inherent work associated with the job. We refer to the inherent size of an elastic job with the random variable $S_E$, and have $S_E \sim Exp(\mu_E)$
We assume that job sizes are unknown to the system, and that inelastic job sizes are exponentially distributed with rate $\mu_I$ while elastic job sizes are exponentially distributed with rate $\mu_E$.
A job's \emph{service rate}, the rate at which work is done on the job in units of work per units of time, is equal to the number of servers on which it runs.
Thus, time required to complete a job of size $x$ on $y$ servers is $\frac{x}{y}$.
Due to the memoryless property of the exponential distribution, we can also describe jobs in terms of a completion rate.
The completion rate of an inelastic job running on $y$ servers is $y\mu_I$ (note that $y \leq$ 1) and the completion rate of an elastic job running on $y$ servers is $y\mu_E$ (where $y \leq k$).

Crucially, we note that the number of servers that a job runs on \emph{does not} change the job's original size or residual size, it simply changes the job's service rate.  It will thus be convenient to do much of our accounting by considering job sizes rather than service rate or completion rate.  We will refer the \emph{total work}, $W$, as the sum of the sizes of all jobs in the system.  Similarly, we will let $W_I$ be the sum of sizes of all inelastic jobs in the system and we will let $W_E$ be the sum of the sizes of all elastic jobs in the system.  We refer to these quantities as the total inelastic work and total elastic work respectively.

We also define analogous quantities describing the number of job in the system.
We let $N$ be the total number of jobs in the system.
We also define $N_I$ to be the total number of inelastic jobs in the system, and define $N_E$ to be the total number of elastic jobs in the system.
Because each job's size is sampled independently of other job sizes, and does not depend on the state of the system, we can relate $N_I$ to $W_I$ and $N_E$ to $W_E$ in expectation.
Specifically,
$$\mathbb{E}[W_I] = \mathbb{E}[N_I]\mathbb{E}[S_I] = \frac{1}{\mu_I}\mathbb{E}[N_I]$$
and
$$\mathbb{E}[W_E] = \mathbb{E}[N_E]\mathbb{E}[S_E] = \frac{1}{\mu_E}\mathbb{E}[N_I].$$
Again, although the service rate of a job might depend on the state of the system, a job's size is independent of the system state, emitting the above identities.
Informally, a job's size can be thought of as the number of core-hours needed to complete the job. Even though an elastic job may complete twice as quickly if it is given 2 servers instead of 1, it still requires the same number of core-hours to complete.
We are simply relating job size (e.g. core-hours) to the number of jobs.

A natural question that emerges in this setup is how to schedule inelastic and elastic jobs on the $k$ servers in order to minimize mean response time. If $\mu_I = \mu_E$ (that is, inelastic jobs and elastic jobs have their sizes distributed according to the same distribution), we know that a strategy called \textbf{Inelastic First (IF)} is optimal. In this work-conserving policy, we always ensure the $k$ servers are working on the maximal number of inelastic jobs possible, filling any idle servers with elastic jobs, if there are any available. Furthermore, jobs within a single class are served first come first serve. What this means for elastic jobs is that (1) only a single elastic job runs at a time, and (2) it uses all servers not used by inelastic jobs. In this writeup, we aim to prove that inelastic first is also optimal for minimizing mean response time when $\mu_I > \mu_E$. \\



